Personas as a Way to Model Truthfulness in Language Models

Large language models (LLMs) are trained on vast amounts of text from the internet, which contains both factual and misleading information about the world. While unintuitive from a classic view of LMs, recent work has shown that the truth value of a statement can be elicited from the model's representations. This paper presents an explanation for why LMs appear to know the truth despite not being trained with truth labels. We hypothesize that the pretraining data is generated by groups of (un)truthful agents whose outputs share common features, and they form a (un)truthful persona. By training on this data, LMs can infer and represent the persona in its activation space. This allows the model to separate truth from falsehoods and controls the truthfulness of its generation. We show evidence for the persona hypothesis via two observations: (1) we can probe whether a model's answer will be truthful before it is generated; (2) finetuning a model on a set of facts improves its truthfulness on unseen topics. Next, using arithmetics as a synthetic environment, we show that structures of the pretraining data are crucial for the model to infer the truthful persona. Overall, our findings suggest that models can exploit hierarchical structures in the data to learn abstract concepts like truthfulness.

==> sections/impact.tex <==
\section*{Impact Statement}

%nj: Seems like this is mandatory for ICML

%Our work tries to understand a mechanism through which LLMs can distinguish between true and false statements --- advancing our understanding of LLMs can both help us predict where they will fail, and demystify the black-box nature of LLM capabilities.
We acknowledge the complexity of the term `truthfulness', especially for subjective/opinionated topics. In this work, we focus on factual questions where experts agree on what is truthful.
Our work aims to understand a mechanism through which LLMs can distinguish true from false statements. Advancing our understanding of LLMs can both help us predict where they will fail, and demystify the black-box nature of LLM capabilities. Also, we hope this work can contribute towards creating more trustworthy LLMs.

